Non-blocking Dynamic Unbounded Graphs with Wait-Free Snapshot

Graphs are arguably one of the most fundamental data-structure used in many domains such as block-chain, networks etc. Theoretically and practically, improving Graph performance is one of the most studied and omnipresent research problems. In this paper, we have implemented a dynamic unbounded concurrent graph which can perform the add, delete or lookup operations on vertices and edges concurrently. All these methods are lock-free and linearizable. On top of this, we have also implemented the wait-free graph snapshot algorithm. To the best of knowledge this is first wait-free implementation of snapshot on concurrent graphs. We have used the snapshot of the algorithm to calculate the diameter and between centrality. We have compared our implementation with its counterparts and outperformed them by a good margin. This illustrates the efficiency of our snapshot method which is a generic method and can be used to perform other useful graph analytics operations.

==> Experiments/Exp1/plot.tex <==
\definecolor{clr1}{RGB}{00,36,92}
\definecolor{clr2}{RGB}{188,80,144}
\definecolor{clr3}{RGB}{255,166,00}
\def \exp_loc{Experiments/Exp1}
\begin{figure}[hbt!]
    \centering
    \caption{Response time with Snapshot}
    \begin{subfigure}[b]{0.45\textwidth}
    
    \begin{tikzpicture}
    \begin{axis}[
    width=\linewidth,
    ybar,
    xlabel={Number of Threads},
    ylabel={Response Time [msec]},
    % xmin=0, xmax=70,
    % ymin=0, ymax=2.5,
    xtick={1,2,3,4,5},
    xticklabels = {13,26,52,78,104},
    % x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    % y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south},
    % ytick={0.5,1.0,1.5,2.0,2.5,3,3.5,4},
    % legend pos=outer north east,
    bar width=4,
    ymajorgrids=true,
    legend entries={\small{REPORT},\small{ICDCN},\small{OPODIS}},
    legend pos=north west,
    legend style={nodes={scale=0.7, transform shape}},
    % grid style=dashed,
]

\addplot[
    color=clr1,
    fill=clr1,
    % mark=square,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_report.csv};
    % coordinates {
    % (1000,0.670373)(1500,1.00508)(2000,1.341778)(2500,1.675643)(3000,2.011006)(3500,2.348578)(4000,2.680916)
    % }
\addplot[
    color=clr2,
    fill=clr2
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_icdcn.csv};
    % coordinates {
    % (1000,0.268939)(1500,0.3985193)(2000,0.552735)(2500,0.679917)(3000,0.818706)(3500,0.963621)(4000,1.090492)
    % };
\addplot[
    color=clr3,
    fill=clr3
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_opodis.csv};

    \end{axis}
    
    \end{tikzpicture}
     \caption[]{Update Intensive}
    \end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}

    \begin{tikzpicture}
    \begin{axis}[
        % width=4.2cm,height=4.5cm,
        width=\linewidth,
        ybar,
        xlabel={Number of Threads},
        % ylabel={Response Time [msec]},
        % xmin=0, xmax=70,
        % ymin=0, ymax=2.5,
         xtick={1,2,3,4,5},
            xticklabels = {13,26,52,78,104},
        % ytick={0.5,1.0,1.5,2.0,2.5,3,3.5,4},
        % legend pos=outer north east,
            bar width=4,
        ymajorgrids=true,
        % grid style=dashed,
    ]
    
    \addplot[
    color=clr1,
    fill=clr1,
    % mark=square,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_report.csv};
    % coordinates {
    % (1000,0.670373)(1500,1.00508)(2000,1.341778)(2500,1.675643)(3000,2.011006)(3500,2.348578)(4000,2.680916)
    % }
\addplot[
    color=clr2,
    fill=clr2
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_icdcn.csv};
    % coordinates {
    % (1000,0.268939)(1500,0.3985193)(2000,0.552735)(2500,0.679917)(3000,0.818706)(3500,0.963621)(4000,1.090492)
    % };
\addplot[
    color=clr3,
    fill=clr3
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_opodis.csv};
        \end{axis}
        \end{tikzpicture}
         \caption{Lookup Intensive}
\end{subfigure}

    
\end{figure}


==> Experiments/Exp2/plot.tex <==
\definecolor{clr1}{RGB}{00,36,92}
\definecolor{clr2}{RGB}{188,80,144}
\definecolor{clr3}{RGB}{255,166,00}
\def \exp_loc{Experiments/Exp2}
\begin{figure}[hbt!]
    \centering
    \caption{Response time with Diameter}
    \begin{subfigure}[b]{0.45\textwidth}
    
    \begin{tikzpicture}
    \begin{axis}[
    width=\linewidth,
    ybar,
    xlabel={Number of Threads},
    ylabel={Response Time [msec]},
    % xmin=0, xmax=70,
    % ymin=0, ymax=2.5,
    xtick={1,2,3,4,5},
    xticklabels = {13,26,52,78,104},
    % x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    % y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south},
    % ytick={0.5,1.0,1.5,2.0,2.5,3,3.5,4},
    % legend pos=outer north east,
    bar width=4,
    ymajorgrids=true,
    legend entries={\small{REPORT},\small{ICDCN},\small{OPODIS}},
    legend pos=north west,
    legend style={nodes={scale=0.7, transform shape}},
    % grid style=dashed,
]

\addplot[
    color=clr1,
    fill=clr1,
    % mark=square,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_report.csv};
    % coordinates {
    % (1000,0.670373)(1500,1.00508)(2000,1.341778)(2500,1.675643)(3000,2.011006)(3500,2.348578)(4000,2.680916)
    % }
\addplot[
    color=clr2,
    fill=clr2
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_icdcn.csv};
    % coordinates {
    % (1000,0.268939)(1500,0.3985193)(2000,0.552735)(2500,0.679917)(3000,0.818706)(3500,0.963621)(4000,1.090492)
    % };
\addplot[
    color=clr3,
    fill=clr3
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_opodis.csv};

    \end{axis}
    
    \end{tikzpicture}
     \caption[]{Update Intensive}
    \end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}

    \begin{tikzpicture}
    \begin{axis}[
        % width=4.2cm,height=4.5cm,
        width=\linewidth,
        ybar,
        xlabel={Number of Threads},
        % ylabel={Response Time [msec]},
        % xmin=0, xmax=70,
        % ymin=0, ymax=2.5,
         xtick={1,2,3,4,5},
            xticklabels = {13,26,52,78,104},
        % ytick={0.5,1.0,1.5,2.0,2.5,3,3.5,4},
        % legend pos=outer north east,
            bar width=4,
        ymajorgrids=true,
        % grid style=dashed,
    ]
    
    \addplot[
    color=clr1,
    fill=clr1,
    % mark=square,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_report.csv};
    % coordinates {
    % (1000,0.670373)(1500,1.00508)(2000,1.341778)(2500,1.675643)(3000,2.011006)(3500,2.348578)(4000,2.680916)
    % }
\addplot[
    color=clr2,
    fill=clr2
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_icdcn.csv};
    % coordinates {
    % (1000,0.268939)(1500,0.3985193)(2000,0.552735)(2500,0.679917)(3000,0.818706)(3500,0.963621)(4000,1.090492)
    % };
\addplot[
    color=clr3,
    fill=clr3
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_opodis.csv};
        \end{axis}
        \end{tikzpicture}
         \caption{Lookup Intensive}
\end{subfigure}

    
\end{figure}


==> Experiments/Exp3/plot.tex <==
\definecolor{clr1}{RGB}{00,36,92}
\definecolor{clr2}{RGB}{188,80,144}
\definecolor{clr3}{RGB}{255,166,00}
\def \exp_loc{Experiments/Exp3}
\begin{figure}[hbt!]
    \centering
    \caption{Response time with Betweeness Centrality}
    \begin{subfigure}[b]{0.45\textwidth}
    
    \begin{tikzpicture}
    \begin{axis}[
    width=\linewidth,
    ybar,
    xlabel={Number of Threads},
    ylabel={Response Time [msec]},
    % xmin=0, xmax=70,
    % ymin=0, ymax=2.5,
    xtick={1,2,3,4,5},
    xticklabels = {13,26,52,78,104},
    % x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    % y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south},
    % ytick={0.5,1.0,1.5,2.0,2.5,3,3.5,4},
    % legend pos=outer north east,
    bar width=4,
    ymajorgrids=true,
    legend entries={\small{REPORT},\small{ICDCN},\small{OPODIS}},
    legend pos=north west,
    legend style={nodes={scale=0.7, transform shape}},
    % grid style=dashed,
]

\addplot[
    color=clr1,
    fill=clr1,
    % mark=square,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_report.csv};
    % coordinates {
    % (1000,0.670373)(1500,1.00508)(2000,1.341778)(2500,1.675643)(3000,2.011006)(3500,2.348578)(4000,2.680916)
    % }
\addplot[
    color=clr2,
    fill=clr2
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_icdcn.csv};
    % coordinates {
    % (1000,0.268939)(1500,0.3985193)(2000,0.552735)(2500,0.679917)(3000,0.818706)(3500,0.963621)(4000,1.090492)
    % };
\addplot[
    color=clr3,
    fill=clr3
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_opodis.csv};

    \end{axis}
    
    \end{tikzpicture}
     \caption[]{Update Intensive}
    \end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}

    \begin{tikzpicture}
    \begin{axis}[
        % width=4.2cm,height=4.5cm,
        width=\linewidth,
        ybar,
        xlabel={Number of Threads},
        % ylabel={Response Time [msec]},
        % xmin=0, xmax=70,
        % ymin=0, ymax=2.5,
         xtick={1,2,3,4,5},
            xticklabels = {13,26,52,78,104},
        % ytick={0.5,1.0,1.5,2.0,2.5,3,3.5,4},
        % legend pos=outer north east,
            bar width=4,
        ymajorgrids=true,
        % grid style=dashed,
    ]
    
    \addplot[
    color=clr1,
    fill=clr1,
    % mark=square,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_report.csv};
    % coordinates {
    % (1000,0.670373)(1500,1.00508)(2000,1.341778)(2500,1.675643)(3000,2.011006)(3500,2.348578)(4000,2.680916)
    % }
\addplot[
    color=clr2,
    fill=clr2
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_icdcn.csv};
    % coordinates {
    % (1000,0.268939)(1500,0.3985193)(2000,0.552735)(2500,0.679917)(3000,0.818706)(3500,0.963621)(4000,1.090492)
    % };
\addplot[
    color=clr3,
    fill=clr3
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_opodis.csv};
        \end{axis}
        \end{tikzpicture}
         \caption{Lookup Intensive}
\end{subfigure}

    
\end{figure}


==> Experiments/Exp4/plot.tex <==
\definecolor{clr1}{RGB}{00,36,92}
\definecolor{clr2}{RGB}{188,80,144}
\definecolor{clr3}{RGB}{255,166,00}
\def \exp_loc{Experiments/Exp4}
\begin{figure}[hbt!]
    \centering
    \caption{Response time with Snapshot}
    \begin{subfigure}[b]{0.45\textwidth}
    
    \begin{tikzpicture}
    \begin{axis}[
    width=\linewidth,
    ybar,
    xlabel={Snapshot Percentage},
    ylabel={Response Time [msec]},
    % xmin=0, xmax=70,
    % ymin=0, ymax=2.5,
    xtick={1,2,3,4,5},
    xticklabels = {2,4,6,8,10},
    % x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    % y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south},
    % ytick={0.5,1.0,1.5,2.0,2.5,3,3.5,4},
    % legend pos=outer north east,
    bar width=4,
    ymajorgrids=true,
    legend entries={\small{REPORT},\small{ICDCN},\small{OPODIS}},
    legend pos=north west,
    legend style={nodes={scale=0.7, transform shape}},
    % grid style=dashed,
]

\addplot[
    color=clr1,
    fill=clr1,
    % mark=square,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_report.csv};
    % coordinates {
    % (1000,0.670373)(1500,1.00508)(2000,1.341778)(2500,1.675643)(3000,2.011006)(3500,2.348578)(4000,2.680916)
    % }
\addplot[
    color=clr2,
    fill=clr2
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_icdcn.csv};
    % coordinates {
    % (1000,0.268939)(1500,0.3985193)(2000,0.552735)(2500,0.679917)(3000,0.818706)(3500,0.963621)(4000,1.090492)
    % };
\addplot[
    color=clr3,
    fill=clr3
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_opodis.csv};

    \end{axis}
    
    \end{tikzpicture}
     \caption[]{Update Intensive}
    \end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}

    \begin{tikzpicture}
    \begin{axis}[
        % width=4.2cm,height=4.5cm,
        width=\linewidth,
        ybar,
        xlabel={Snapshot Percentage},
        % ylabel={Response Time [msec]},
        % xmin=0, xmax=70,
        % ymin=0, ymax=2.5,
         xtick={1,2,3,4,5},
            xticklabels ={2,4,6,8,10},
        % ytick={0.5,1.0,1.5,2.0,2.5,3,3.5,4},
        % legend pos=outer north east,
            bar width=4,
        ymajorgrids=true,
        % grid style=dashed,
    ]
    
    \addplot[
    color=clr1,
    fill=clr1,
    % mark=square,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_report.csv};
    % coordinates {
    % (1000,0.670373)(1500,1.00508)(2000,1.341778)(2500,1.675643)(3000,2.011006)(3500,2.348578)(4000,2.680916)
    % }
\addplot[
    color=clr2,
    fill=clr2
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_icdcn.csv};
    % coordinates {
    % (1000,0.268939)(1500,0.3985193)(2000,0.552735)(2500,0.679917)(3000,0.818706)(3500,0.963621)(4000,1.090492)
    % };
\addplot[
    color=clr3,
    fill=clr3
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_opodis.csv};
        \end{axis}
        \end{tikzpicture}
         \caption{Lookup Intensive}
\end{subfigure}

    
\end{figure}


==> Experiments/Exp5/plot.tex <==
\definecolor{clr1}{RGB}{00,36,92}
\definecolor{clr2}{RGB}{188,80,144}
\definecolor{clr3}{RGB}{255,166,00}
\def \exp_loc{Experiments/Exp5}
\begin{figure}[hbt!]
    \centering
    \caption{Response time with Diameter}
    \begin{subfigure}[b]{0.45\textwidth}
    
    \begin{tikzpicture}
    \begin{axis}[
    width=\linewidth,
    ybar,
    xlabel={Snapshot Percentage},
    ylabel={Response Time [msec]},
    % xmin=0, xmax=70,
    % ymin=0, ymax=2.5,
    xtick={1,2,3,4,5},
    xticklabels = {2,4,6,8,10},
    % x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    % y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south},
    % ytick={0.5,1.0,1.5,2.0,2.5,3,3.5,4},
    % legend pos=outer north east,
    bar width=4,
    ymajorgrids=true,
    legend entries={\small{REPORT},\small{ICDCN},\small{OPODIS}},
    legend pos=north west,
    legend style={nodes={scale=0.7, transform shape}},
    % grid style=dashed,
]

\addplot[
    color=clr1,
    fill=clr1,
    % mark=square,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_report.csv};
    % coordinates {
    % (1000,0.670373)(1500,1.00508)(2000,1.341778)(2500,1.675643)(3000,2.011006)(3500,2.348578)(4000,2.680916)
    % }
\addplot[
    color=clr2,
    fill=clr2
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_icdcn.csv};
    % coordinates {
    % (1000,0.268939)(1500,0.3985193)(2000,0.552735)(2500,0.679917)(3000,0.818706)(3500,0.963621)(4000,1.090492)
    % };
\addplot[
    color=clr3,
    fill=clr3
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_opodis.csv};

    \end{axis}
    
    \end{tikzpicture}
     \caption[]{Update Intensive}
    \end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}

    \begin{tikzpicture}
    \begin{axis}[
        % width=4.2cm,height=4.5cm,
        width=\linewidth,
        ybar,
        xlabel={Snapshot Percentage},
        % ylabel={Response Time [msec]},
        % xmin=0, xmax=70,
        % ymin=0, ymax=2.5,
         xtick={1,2,3,4,5},
            xticklabels ={2,4,6,8,10},
        % ytick={0.5,1.0,1.5,2.0,2.5,3,3.5,4},
        % legend pos=outer north east,
            bar width=4,
        ymajorgrids=true,
        % grid style=dashed,
    ]
    
    \addplot[
    color=clr1,
    fill=clr1,
    % mark=square,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_report.csv};
    % coordinates {
    % (1000,0.670373)(1500,1.00508)(2000,1.341778)(2500,1.675643)(3000,2.011006)(3500,2.348578)(4000,2.680916)
    % }
\addplot[
    color=clr2,
    fill=clr2
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_icdcn.csv};
    % coordinates {
    % (1000,0.268939)(1500,0.3985193)(2000,0.552735)(2500,0.679917)(3000,0.818706)(3500,0.963621)(4000,1.090492)
    % };
\addplot[
    color=clr3,
    fill=clr3
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_opodis.csv};
        \end{axis}
        \end{tikzpicture}
         \caption{Lookup Intensive}
\end{subfigure}

    
\end{figure}


==> Experiments/Exp6/plot.tex <==
\definecolor{clr1}{RGB}{00,36,92}
\definecolor{clr2}{RGB}{188,80,144}
\definecolor{clr3}{RGB}{255,166,00}
\def \exp_loc{Experiments/Exp6}
\begin{figure}[hbt!]
    \centering
    \caption{Response time with Betweeness Centrality}
    \begin{subfigure}[b]{0.45\textwidth}
    
    \begin{tikzpicture}
    \begin{axis}[
    width=\linewidth,
    ybar,
    xlabel={Snapshot Percentage},
    ylabel={Response Time [msec]},
    % xmin=0, xmax=70,
    % ymin=0, ymax=2.5,
    xtick={1,2,3,4,5},
    xticklabels={2,4,6,8,10},
    % x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    % y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south},
    % ytick={0.5,1.0,1.5,2.0,2.5,3,3.5,4},
    % legend pos=outer north east,
    bar width=4,
    ymajorgrids=true,
    legend entries={\small{REPORT},\small{ICDCN},\small{OPODIS}},
    legend pos=north west,
    legend style={nodes={scale=0.7, transform shape}},
    % grid style=dashed,
]

\addplot[
    color=clr1,
    fill=clr1,
    % mark=square,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_report.csv};
    % coordinates {
    % (1000,0.670373)(1500,1.00508)(2000,1.341778)(2500,1.675643)(3000,2.011006)(3500,2.348578)(4000,2.680916)
    % }
\addplot[
    color=clr2,
    fill=clr2
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_icdcn.csv};
    % coordinates {
    % (1000,0.268939)(1500,0.3985193)(2000,0.552735)(2500,0.679917)(3000,0.818706)(3500,0.963621)(4000,1.090492)
    % };
\addplot[
    color=clr3,
    fill=clr3
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/up_opodis.csv};

    \end{axis}
    
    \end{tikzpicture}
     \caption[]{Update Intensive}
    \end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}

    \begin{tikzpicture}
    \begin{axis}[
        % width=4.2cm,height=4.5cm,
        width=\linewidth,
        ybar,
        xlabel={Snapshot Percentage},
        % ylabel={Response Time [msec]},
        % xmin=0, xmax=70,
        % ymin=0, ymax=2.5,
         xtick={1,2,3,4,5},
        xticklabels={2,4,6,8,10},
        % ytick={0.5,1.0,1.5,2.0,2.5,3,3.5,4},
        % legend pos=outer north east,
            bar width=4,
        ymajorgrids=true,
        % grid style=dashed,
    ]
    
    \addplot[
    color=clr1,
    fill=clr1,
    % mark=square,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_report.csv};
    % coordinates {
    % (1000,0.670373)(1500,1.00508)(2000,1.341778)(2500,1.675643)(3000,2.011006)(3500,2.348578)(4000,2.680916)
    % }
\addplot[
    color=clr2,
    fill=clr2
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_icdcn.csv};
    % coordinates {
    % (1000,0.268939)(1500,0.3985193)(2000,0.552735)(2500,0.679917)(3000,0.818706)(3500,0.963621)(4000,1.090492)
    % };
\addplot[
    color=clr3,
    fill=clr3
    % mark=Mercedes star flipped,
    ]
    table[ignore chars={(,)},col sep=comma] {\exp_loc/look_opodis.csv};
        \end{axis}
        \end{tikzpicture}
         \caption{Lookup Intensive}
\end{subfigure}

    
\end{figure}


==> Experiments/Result1.tex <==
\begin{figure*}[h!]
\captionsetup[subfigure]{justification=centering}
\centering
  \includegraphics[width = 0.80\linewidth]{Plots/legend_SSS.png}
  \subfloat[]{  \includegraphics[width=0.33\linewidth]{Plots/Read Heavy Snapshot.pdf}}
   \subfloat[]{ 
  \includegraphics[width=0.33\linewidth]{Plots/Read Heavy Diameter.pdf}}
  % \vspace{1em}
    \subfloat[]{ 
    	\includegraphics[width=0.33\linewidth]{Plots/Read Heavy Betweeness Centrality.pdf}}
\vspace{1em}
    \subfloat[]{ 
  \includegraphics[width=0.33\linewidth]{Plots/Update Heavy Snapshot.pdf}}
  % \vspace{1em}
   \subfloat[]{ 
  \includegraphics[width=0.33\linewidth]{Plots/Update Heavy Diameter.pdf}}
   \subfloat[]{ 
  \includegraphics[width=0.33\linewidth]{Plots/Update Heavy Betweeness Centrality.pdf}}
    % \subfloat[]{ 
  % \includegraphics[width=0.24\linewidth]{Diagram/Read_Heavy_LLC_Misses.pdf}}
   % \subfloat[]{ 
  % \includegraphics[width=0.24\linewidth]{Diagram/Update_Heavy_LLC_Misses.pdf}}
\caption{Performance of our implementation when compared with its counterparts. x-axis: Number of threads. y-axis: Time taken in microseconds. (a) Read Heavy workload with snapshot, (b) Read Heavy workload with Diameter, (c) Read Heavy workload with Betweenness Centrality, (d) Update Heavy with snapshot, (e) Update Heavy with Diameter, (f) Update Heavy with Betweenness Centrality.}
% \caption{The performance of \textbf{Kanva} when compared to different datastrucutre. (a) read heavy workload with uniform dataset (b) read Heavy workload with different datasets (1: uniform, 2: normal, 3: Amazon, 4: Facebook, 5: OSM (Open Street Map), 6: Wikipedia) with 64 threads (c) update heavy Workload with uniform dataset (d) update heavy workload with different datasets  with 64 threads (e) YCSB (A: update-heavy, B: read-heavy, C: read-only) workloads with uniform distribution (f) YCSB workloads with zipfian distribution (g) last-level cache misses (lower is better) on read heavy workload, (h) last level cache misses on update heavy workload}
\label{fig:results1}
\end{figure*}

==> Experiments/Result2.tex <==
\begin{figure*}[h!]
\captionsetup[subfigure]{justification=centering}
\centering
  \includegraphics[width = 0.80\linewidth]{Plots/legend_SSS.png}
  \subfloat[]{  \includegraphics[width=0.33\linewidth]{Plots/Read Heavy with varying Snapshot.pdf}}
   \subfloat[]{ 
  \includegraphics[width=0.33\linewidth]{Plots/Read Heavy with varying Diameter.pdf}}
  % \vspace{1em}
    \subfloat[]{ 
    	\includegraphics[width=0.33\linewidth]{Plots/Read Heavy with varying Betweeness Centrality.pdf}}
\vspace{1em}
    \subfloat[]{ 
  \includegraphics[width=0.33\linewidth]{Plots/Update Heavy with varying Snapshot.pdf}}
  % \vspace{1em}
   \subfloat[]{ 
  \includegraphics[width=0.33\linewidth]{Plots/Update Heavy with varying Diameter.pdf}}
   \subfloat[]{ 
  \includegraphics[width=0.33\linewidth]{Plots/Update Heavy with varying Betweeness Centrality.pdf}}
    % \subfloat[]{ 
  % \includegraphics[width=0.24\linewidth]{Diagram/Read_Heavy_LLC_Misses.pdf}}
   % \subfloat[]{ 
  % \includegraphics[width=0.24\linewidth]{Diagram/Update_Heavy_LLC_Misses.pdf}}
\caption{Performance of our implementation with varying percentage of graph analytics operation. x-axis: \%age of graph analytics operations. y-axis: Time taken in micro seconds. (a) Read Heavy workload with snapshot, (b) Read Heavy workload with Diameter, (c) Read Heavy workload with Betweeness Centrality, (d) Update Heavy with snapshot, (e) Update Heavy with Diameter, (f) Update Heavy with Betweeness Centrality.}
% \caption{The performance of \textbf{Kanva} when compared to different datastrucutre. (a) read heavy workload with uniform dataset (b) read Heavy workload with different datasets (1: uniform, 2: normal, 3: Amazon, 4: Facebook, 5: OSM (Open Street Map), 6: Wikipedia) with 64 threads (c) update heavy Workload with uniform dataset (d) update heavy workload with different datasets  with 64 threads (e) YCSB (A: update-heavy, B: read-heavy, C: read-only) workloads with uniform distribution (f) YCSB workloads with zipfian distribution (g) last-level cache misses (lower is better) on read heavy workload, (h) last level cache misses on update heavy workload}
\label{fig:results1}
\end{figure*}

==> experiment.tex <==
\input{Experiments/Result1}
\paragraph{Platform Configuration:}
We conducted our experiments on a system with Intel(R) Xeon(R) Gold 6230R CPU packing 52 cores with a clock speed of 2.10GHz. There are 2 logical threads for each core, each with a private 32KB L1 and 1024KB L2 cache. The 36608KB L3 cache is shared across the cores. The system has 376GB of RAM and 1TB of  hard disk. It runs on a 64-bit Linux operating system. 
\input{Experiments/Result2}
\paragraph{Experimental Setup:}All implementations are in C++ without garbage collection. We used Posix threads for multi-threaded implementation. We initially populate the graph with a fixed set of nodes and edges and then spawn the required set of threads(13,26,52, 78, and 108). There are six basic operations, namely contains, insert and delete on nodes/edges, and one critical operation, which would be either snapshot/ diameter /betweenness centrality. Each thread will execute for at least t secs. During the execution, each thread would select the next operation based on the workload. Thus all the threads combined will perform n such operations within t secs. The evaluation metric used is Average Time, for which we consider the Average Time taken to complete each operation. We measure the Average Time w.r.t (i). Increasing spawned threads (ii) Increasing the workload to critical operations(Snapshot/Diameter/Betweenness Centrality) (iii) Multiple Snap graph Datasets.
\paragraph{Workload Distribution :}The distribution is over the following ordered set of Operations (AddVertex, RemoveVertex, ContainsVertex, AddEdge, RemoveEdge, ContainsEdge, and Critical Operation(Snapshot/Diameter/Betweenness Centrality). 
\begin{enumerate}
    \item Read Heavy Workload : 3\%, 2\%, 45\%, 3\%, 2\%, 45\% , 2\%
    \item Update Heavy Workload: 12\%, 13\%, 25\%, 13\%, 12\%, 25\% , 2\%
\end{enumerate}
In one of the experiments we measure the Average Time against the following Critical Section Workload : (2\%, 4\%, 6\%, 8\%, and 10\%), in which case we reduce the ContainsEdge and ContainsVertex workload by the same factor.

\paragraph{Algorithms :} We compare our wait-free Snapshot/Diameter/Betweenness Centrality approaches to the obstruction-free implementation of the same operations using Chatterjee et al. \cite{Chatterjee+:NbGraph:ICDCN-19} , 
and Chatterjee et al. \cite{Chatterjee2021NonBlockingDU}. We have named them \ICDCN and Panigraham, respectively, and our approach as \reports.
\paragraph{Performance for various Graph Analytics Operation}In Fig 5. we compare the Average times of the algorithms under the two different workloads mentioned above. Initially, with Snapshot, and then we replace the Snapshot operation with Diameter and Betweenness Centrality(BC). In the case of Snapshot, our algorithm performs considerably better than others. This happens because, in our case, if a new thread needs to perform Snapshot, it helps the existing Snapshot if present. Thus we see that the Average Time remains the same even with increasing active threads as more threads will be involved in creating a snapshot.
On the other hand, in the obstruction-free algorithm, each thread creates its own independent Snapshot. The diameter and BC are performed independently using Snapshot by each thread in all three algorithms. Hence we see the Average time increasing with threads, but still, \reports perform better.

In Fig 6, we increase the Snapshot percentage as explained in the workload distribution section on both read-heavy and update-heavy workloads. We perform the same experiment by replacing the Snapshot operation with Diameter and Betweenness Centrality. We see that the performance of the \reports is far better than the other obstruction-free approaches. The Average time in the case of Snapshot is not affected by the increase in workload. Although Snapshot is the slowest operation, increasing its workload should increase the Average time, but as more threads would be involved in constructing the Snapshot, it would take less time to complete it. Hence, we see the Average time reducing in some cases, but overall, it remains almost the same. 

==> results.tex <==
\input{Experiments/Exp1/plot}
\input{Experiments/Exp2/plot}
\input{Experiments/Exp3/plot}
\input{Experiments/Exp4/plot}
\input{Experiments/Exp5/plot}
\input{Experiments/Exp6/plot}
